A Platform for Ultra-fast Proton Probing of Matter in Extreme Conditions

Recent development of Ultra short and Intense laser system paved the way for the generation of short and brilliant proton sources that can be used to study plasmas at extreme conditions in the context of High Energy Density physics. Energy selection, focusing and transport of such sources is still a challenge that is not completely solved. here we present a novel and simple design for a isochrone magnetic selector capable of angular and energy selection of proton sources by drastically reducing the temporal spread if compared with the state of the art. The isochrone selector is demanded for studying proton stopping power in Warm Dense Matter close to the Bragg peak (proton energy below 1 MeV) where the reduced investigated masses imply a short plasma stagnation time ($<$ 100 ps). The proposed selector can also be used at higher proton energy by pushing the final time spread at the level of few ps with important implications for the study of coherent energy deposition in biology and medical physics. Analytical estimations and Monte Carlo simulations are presented to validate the proposed configurations.

==> references.tex <==

	\bibitem{Hur19}
	\bibinfo{author}{Hurricane, O.} \emph{et~al.}
	\newblock \bibinfo{title}{{Approaching a burning plasma on the NIF}}.
	\newblock \emph{\bibinfo{journal}{Phys. Plasmas}}
	\textbf{\bibinfo{volume}{26}}, \bibinfo{pages}{052704}
	(\bibinfo{year}{2019}).
	
	\bibitem{Zyl19a}
	\bibinfo{author}{Zylstra, A.} \emph{et~al.}
	\newblock \bibinfo{title}{{On alpha-particle transport in inertial fusion}}.
	\newblock \emph{\bibinfo{journal}{Phys. Plasmas}}
	\textbf{\bibinfo{volume}{26}}, \bibinfo{pages}{800--806}
	(\bibinfo{year}{2019}).
	
	%\bibitem{Hur16}
	%\bibinfo{author}{{Hurricane}, O.~A.} \emph{et~al.}
	%\newblock \bibinfo{title}{{Inertially confined fusion plasmas %dominated by
	%		alpha-particle self-heating}}.
	%\newblock \emph{\bibinfo{journal}{Nature Physics}}
	%\textbf{\bibinfo{volume}{12}}, \bibinfo{pages}{800--806}
	%(\bibinfo{year}{2016}).
	
	\bibitem{Cal00}
	\bibinfo{author}{{Callahan-Miller}, D.~A.} \& \bibinfo{author}{{Tabak}, M.}
	\newblock \bibinfo{title}{{Progress in target physics and design for heavy ion
			fusion}}.
	\newblock \emph{\bibinfo{journal}{Phys. Plasmas}}
	\textbf{\bibinfo{volume}{7}}, \bibinfo{pages}{2083--2091}
	(\bibinfo{year}{2000}).
	
	\bibitem{Hof18}
	\bibinfo{author}{{Hofmann}, I.} \emph{et~al.}
	\newblock \bibinfo{title}{{Review of accelerator driven heavy ion nuclear fusion}}.
	\newblock \emph{\bibinfo{journal}{Matter Radiat. at Extremes}}
	\textbf{\bibinfo{volume}{3}}, \bibinfo{pages}{1-11}
	(\bibinfo{year}{2018}).
		
	\bibitem{Rot01}
	\bibinfo{author}{{Roth}, M.} \emph{et~al.}
	\newblock \bibinfo{title}{{Fast Ignition by Intense Laser-Accelerated Proton Beams}}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. Lett.}}
	\textbf{\bibinfo{volume}{86}}, \bibinfo{pages}{436--439}
	(\bibinfo{year}{2001}).
	
	\bibitem{Fer14}
	\bibinfo{author}{{Fern{\'a}ndez}, J.~C.} \emph{et~al.}
	\newblock \bibinfo{title}{{Fast ignition with laser-driven proton and ion beams}}.
	\newblock \emph{\bibinfo{journal}{Nucl. Fusion}}
	\textbf{\bibinfo{volume}{54}}, \bibinfo{pages}{054006}
	(\bibinfo{year}{2014}).
	
	\bibitem{Kim15}
	\bibinfo{author}{{Kim}, J.} \emph{et~al.}
	\newblock \bibinfo{title}{{Self-Consistent Simulation of Transport and Energy Deposition of Intense Laser-Accelerated Proton Beams in Solid-Density Matter}}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. Lett.}}
	\textbf{\bibinfo{volume}{115}}, \bibinfo{pages}{054801}
	(\bibinfo{year}{2015}).
	
	\bibitem{Kim18}
	\bibinfo{author}{{Kim}, J.} \emph{et~al.}
	\newblock \bibinfo{title}{{Anomalous material-dependent transport of focused, laser-driven proton beams}}.
	\newblock \emph{\bibinfo{journal}{Sci. Rep.}}
	\textbf{\bibinfo{volume}{8}}, \bibinfo{pages}{17538}
	(\bibinfo{year}{2018}).
	
	\bibitem{Sha16}
	\bibinfo{author}{{Sharkov}, B.} \emph{et~al.}
	\newblock \bibinfo{title}{{High energy density physics with intense ion beams}}.
	\newblock \emph{\bibinfo{journal}{Matter Radiat. at Extremes}}
	\textbf{\bibinfo{volume}{1}}, \bibinfo{pages}{28-47}
	(\bibinfo{year}{2016}).
	
	\bibitem{Pat03}
	\bibinfo{author}{{Patel}, P.} \emph{et~al.}
	\newblock \bibinfo{title}{{Isochoric Heating of Solid-Density Matter with an Ultrafast Proton Beam}}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. Lett.}}
	\textbf{\bibinfo{volume}{91}}, \bibinfo{pages}{125004}
	(\bibinfo{year}{2003}).

	\bibitem{McG20}
	\bibinfo{author}{{McGuffey}, C.} \emph{et~al.}
	\newblock \bibinfo{title}{{Focussing Protons from a Kilojoule Laser for Intense Beam Heating using Proximal Target Structures}}.
	\newblock \emph{\bibinfo{journal}{Sci. Rep.}}
	\textbf{\bibinfo{volume}{10}}, \bibinfo{pages}{9415}
	(\bibinfo{year}{2020}).
	
	\bibitem{Man10}
	\bibinfo{author}{{Mancic}, A.} \emph{et~al.}
	\newblock \bibinfo{title}{Picosecond Short-Range Disordering in Isochorically Heated Aluminum at Solid Density}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. Lett.}}
	\textbf{\bibinfo{volume}{104}}, \bibinfo{pages}{035002}
	(\bibinfo{year}{2010}).
	

	
	\bibitem{Pin19}
	\bibinfo{author}{{Ping}, Y.} \emph{et~al.}
	\newblock \bibinfo{title}{{Heat-release equation of state and thermal conductivity of warm dense carbon by proton differential heating}}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. E}}
	\textbf{\bibinfo{volume}{100}}, \bibinfo{pages}{043204}
	(\bibinfo{year}{2019}).
	
	\bibitem{Gra20}
	\bibinfo{author}{{Grabowski}, P.~E.} \emph{et~al.}
	\newblock \bibinfo{title}{{Review of the first charged-particle transport coefficient comparison workshop}}.
	\newblock \emph{\bibinfo{journal}{High Energy Density Phys.}}
	\textbf{\bibinfo{volume}{37}}, \bibinfo{pages}{100905}
	(\bibinfo{year}{2020}).
	
	\bibitem{McK17}
	\bibinfo{author}{{McKelvey}, A.} \emph{et~al.}
	\newblock \bibinfo{title}{{Thermal conductivity measurements of proton-heated warm dense aluminum}}.
	\newblock \emph{\bibinfo{journal}{Sci. Rep.}}
	\textbf{\bibinfo{volume}{7}}, \bibinfo{pages}{7015}
	(\bibinfo{year}{2017}).
	
	\bibitem{Whi12}
	\bibinfo{author}{{White}, T.} \emph{et~al.}
	\newblock \bibinfo{title}{{Observation of inhibited electron-ion coupling in strongly heated graphite}}.
	\newblock \emph{\bibinfo{journal}{Sci. Rep.}}
	\textbf{\bibinfo{volume}{2}}, \bibinfo{pages}{889}
	(\bibinfo{year}{2012}).
	
	\bibitem{Mac06}
	\bibinfo{author}{{Mackinnon}, A.} \emph{et~al.}
	\newblock \bibinfo{title}{{Proton Radiography of a Laser-Driven Implosion}}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. Lett.}}
	\textbf{\bibinfo{volume}{97}}, \bibinfo{pages}{045001}
	(\bibinfo{year}{2006}).

	\bibitem{Vol11}
	\bibinfo{author}{{Volpe}, L.} \emph{et~al.}
	\newblock \bibinfo{title}{{Proton radiography of laser-driven imploding target in cylindrical geometry}}.
	\newblock \emph{\bibinfo{journal}{Phys. Plasmas}}
	\textbf{\bibinfo{volume}{18}}, \bibinfo{pages}{012704}
	(\bibinfo{year}{2011}).
	
	%----------------------------------------------------------------------------------------
    % INTRODUCTION: EXPERIMENTS AND MODELS
    %----------------------------------------------------------------------------------------
	
	\bibitem{Hof90}
	\bibinfo{author}{{Hoffmann}, D.~H.~H.} \emph{et~al.}
	\newblock \bibinfo{title}{{Energy loss of heavy ions in a plasma target}}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. A}}
	\textbf{\bibinfo{volume}{42}}, \bibinfo{pages}{2313--2321}
	(\bibinfo{year}{1990}).
	
	\bibitem{Die90}
	\bibinfo{author}{{Dietrich}, K.-G.} \emph{et~al.}
	\newblock \bibinfo{title}{{Energy loss of heavy ions in a dense hydrogen plasma}}.
	\newblock \emph{\bibinfo{journal}{Z. Phys. D Atoms Molec. Clust.}} \textbf{\bibinfo{volume}{16}}, \bibinfo{pages}{229--230}
	(\bibinfo{year}{1990}).
	
	\bibitem{Bel96}
	\bibinfo{author}{{Belyaev}, G.}  \emph{et~al.}
	\newblock \bibinfo{title}{{Measurement of the Coulomb energy loss by fast protons in a plasma target}}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. E}}
	\textbf{\bibinfo{volume}{53}}, \bibinfo{pages}{2701}
	(\bibinfo{year}{1996}).
	
	\bibitem{Fra13}
	\bibinfo{author}{{Frank}, A.} \emph{et~al.}
	\newblock \bibinfo{title}{{Energy Loss and Charge Transfer of Argon in a Laser-Generated Carbon Plasma}}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. Lett.}}
	\textbf{\bibinfo{volume}{110}}, \bibinfo{pages}{115001}
	(\bibinfo{year}{2013}).
	
	\bibitem{Ger03}
	\bibinfo{author}{{Gericke}, D.~O.} \& \bibinfo{author}{{Schlanges}, M.}
	\newblock \bibinfo{title}{{Energy deposition of heavy ions in the regime of strong beam-plasma correlations}}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. E}}
	\textbf{\bibinfo{volume}{67}}, \bibinfo{pages}{037401}
	(\bibinfo{year}{2003}).
	
	\bibitem{Cay15}
	\bibinfo{author}{Cayzac, W.} \emph{et~al.}
	\newblock \bibinfo{title}{Predictions for the energy loss of light ions in laser-generated plasmas at low and medium velocities}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. E}}
	\textbf{\bibinfo{volume}{92}}, \bibinfo{pages}{053109}
	(\bibinfo{year}{2015}).
	
	\bibitem{Cay17}
	\bibinfo{author}{Cayzac, W.} \emph{et~al.}
	\newblock \bibinfo{title}{Experimental discrimination of ion stopping models near the Bragg peak in highly ionized matter}.
	\newblock \emph{\bibinfo{journal}{Nat. Commun.}}
	\textbf{\bibinfo{volume}{8}}, \bibinfo{pages}{15693}
	(\bibinfo{year}{2017}).
	
	\bibitem{Fre19}
	\bibinfo{author}{Frenje, J.~A.} \emph{et~al.}
	\newblock \bibinfo{title}{Experimental Validation of Low-Z Ion-Stopping Formalisms around the Bragg Peak in High-Energy-Density Plasmas}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. Lett.}}
	\textbf{\bibinfo{volume}{122}}, \bibinfo{pages}{015002}
	(\bibinfo{year}{2019}).
	
	\bibitem{Ger02b}
	\bibinfo{author}{{Gericke}, D.~O.} \emph{et~al.}
	\newblock \bibinfo{title}{{Stopping power of nonideal, partially ionized plasmas}}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. E}}
	\textbf{\bibinfo{volume}{65}}, \bibinfo{pages}{036406}
	(\bibinfo{year}{2002}).
	
	\bibitem{Edi13}
	\bibinfo{author}{{Edie}, D.~J.}  \emph{et~al.}
	\newblock \bibinfo{title}{{{$\alpha$}-particle stopping and electron-ion energy
			relaxation in highly compressed ICF fuel}}.
	\newblock In \emph{\bibinfo{booktitle}{Eur. Phys. J. Web Conferences}}, vol.~\bibinfo{volume}{59}, \bibinfo{pages}{5018}
	(\bibinfo{year}{2013}).
	
	\bibitem{Deu14}
	\bibinfo{author}{{Deutsch}, C.} \emph{et~al.}
	\newblock \bibinfo{title}{{Multiple scattering in electron fluid and energy loss in multi-ionic targets}}.
	\newblock \emph{\bibinfo{journal}{Nucl. Instrum. Methods Phys. Res. A}}
	\textbf{\bibinfo{volume}{733}}, \bibinfo{pages}{39--44}
	(\bibinfo{year}{2014}).
	
	\bibitem{Din18}
	\bibinfo{author}{{Ding}, Y.~H.} \emph{et~al.}
	\newblock \bibinfo{title}{Ab Initio Studies on the Stopping Power of Warm Dense Matter with Time-Dependent Orbital-Free Density Functional Theory}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. Lett.}}
	\textbf{\bibinfo{volume}{121}}, \bibinfo{pages}{145001}
	(\bibinfo{year}{2018}).
	
	\bibitem{Whi18}
	\bibinfo{author}{{White}, A.~J.} \emph{et~al.}
	\newblock \bibinfo{title}{Time-dependent orbital-free density functional theory for electronic stopping power: Comparison to the Mermin-Kohn-Sham theory at high temperatures}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. B}}
	\textbf{\bibinfo{volume}{98}}, \bibinfo{pages}{144302}
	(\bibinfo{year}{2018}).
	
	\bibitem{Hay15}
	\bibinfo{author}{{Hayes}, A.~C.} \emph{et~al.}
	\newblock \bibinfo{title}{{Reaction-in-flight neutrons as a test of stopping power in degenerate plasmas}}.
	\newblock \emph{\bibinfo{journal}{Phys. Plasmas}}
	\textbf{\bibinfo{volume}{22}}, \bibinfo{pages}{082703}
	(\bibinfo{year}{2015}).
	
	\bibitem{Hay20}
	\bibinfo{author}{{Hayes}, A.~C.} \emph{et~al.}
	\newblock \bibinfo{title}{{Plasma stopping-power measurements reveal transition from non-degenerate to degenerate plasmas}}.
	\newblock \emph{\bibinfo{journal}{Nat. Phys.}}
	\textbf{\bibinfo{volume}{16}}, \bibinfo{pages}{432--437}
	(\bibinfo{year}{2020}).
	
	\bibitem{Zyl15}
	\bibinfo{author}{Zylstra, A.~B.} \emph{et~al.}
	\newblock \bibinfo{title}{Measurement of charged-particle stopping in warm dense plasma}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. Lett.}}
	\textbf{\bibinfo{volume}{114}}, \bibinfo{pages}{215002}
	(\bibinfo{year}{2015}).
	
	\bibitem{Che18}
	\bibinfo{author}{{Chen, S.~N.}} \emph{et~al.}
	\newblock \bibinfo{title}{Experimental evidence for the enhanced and reduced stopping regimes for protons propagating through hot plasmas}.
	\newblock \emph{\bibinfo{journal}{Sci. Rep.}
	\textbf{\bibinfo{volume}{8}}, \bibinfo{pages}{14586}
	(\bibinfo{year}{2018})}.
	
	\bibitem{Ren20}
	\bibinfo{author}{{Ren, J.}} \emph{et~al.}
	\newblock \bibinfo{title}{Observation of a high degree of stopping for laser-accelerated intense proton beams in dense ionized matter}.
	\newblock \emph{\bibinfo{journal}{Nat. Commun.}
	\textbf{\bibinfo{volume}{11}}, \bibinfo{pages}{5157}
	(\bibinfo{year}{2020})}.
	
	\bibitem{Zyl20}
	\bibinfo{author}{{Zylstra, A.~B.}} \emph{et~al.}
	\newblock \bibinfo{title}{Platform development for dE/dx measurements on short-pulse laser facilities}.
	\newblock \emph{\bibinfo{journal}{High Energy Density Phys.}
	\textbf{\bibinfo{volume}{35}}, \bibinfo{pages}{100731}
	(\bibinfo{year}{2020})}.
	
	\bibitem{Jah19}
	\bibinfo{author}{{Jahn, D.}} \emph{et~al.}
	\newblock \bibinfo{title}{Focusing of multi-MeV, subnanosecond proton bunches from a laser-driven source}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. Accel. Beams}
	\textbf{\bibinfo{volume}{22}}, \bibinfo{pages}{011301}
	(\bibinfo{year}{2019})}.
	
	%----------------------------------------------------------
	% RESULTS: SETUP AND MODELLING PART
	%----------------------------------------------------------

	\bibitem{Vol19}
	\bibinfo{author}{{Volpe}, L.}, 
	\bibinfo{author}{{Fedosejevs}, R.},
	\bibinfo{author}{{Gatti}, G.}, 
	\bibinfo{author}{{Pérez-Hernández}, J.~A.},
	\bibinfo{author}{{Méndez}, C.}, \bibinfo{author}{{Apiñaniz},J.},
	\bibinfo{author}{{Vaisseau},X.},
	\bibinfo{author}{{Salgado}, C.}, 
	\bibinfo{author}{{Huault}, M.}
	\bibinfo{author}{{Malko}, S.}
	\bibinfo{author}{{Zeraouli}, G.}
	\bibinfo{author}{{Ospina}, V.}
	\bibinfo{author}{{Longman}, A.}
	\bibinfo{author}{{De Luis}, D.}
	\bibinfo{author}{{Li}, K.}
	\bibinfo{author}{{Varela}, O.}
	\bibinfo{author}{{García}, E.}
	\bibinfo{author}{{Hernández}, I.}
	\bibinfo{author}{{Pisonero}, J.}
	\bibinfo{author}{{García Ajates}, J.}
	\bibinfo{author}{{Alvarez}, J.}
	\bibinfo{author}{{García}, C.}
	\bibinfo{author}{{Rico}, M.}
	\bibinfo{author}{{Arana}, D.}
	\bibinfo{author}{{ Hernández-Toro}, J.}
	\&
	\bibinfo{author}{{Roso}, L.}
	\newblock \bibinfo{title}{{Generation of high energy laser-driven electron and proton sources with the 200 TW system VEGA 2 at the Centro de Laseres Pulsados}}.
	\newblock \emph{\bibinfo{journal}{High Power Laser Sci. Eng.}} \textbf{\bibinfo{volume}{7}}, \bibinfo{pages}{25}
	(\bibinfo{year}{2019}).
	
	\bibitem{Wil01}
	\bibinfo{author}{{Wilks}, S.}, 
	\bibinfo{author}{{Langdon,}, A.},
	\bibinfo{author}{{Cowan}, T.}, 
	\bibinfo{author}{{Roth}, M.},
	\bibinfo{author}{{Singh}, M.}, \bibinfo{author}{{Hatchett}, S.},
	\bibinfo{author}{{Key},M.~H.},
	\bibinfo{author}{{Pennington}, D.}, \bibinfo{author}{{MacKinnon}, A.}
	\&
	\bibinfo{author}{{Snavely}, R.}
	\newblock \bibinfo{title}{{Energetic proton generation in ultra-intense laser–solid interactions}}.
	\newblock \emph{\bibinfo{journal}{Phys. Plasmas}} \textbf{\bibinfo{volume}{8}}, \bibinfo{pages}{542}
	(\bibinfo{year}{2001}).
	
	\bibitem{Api21}
	\bibinfo{author}{{Apiñaniz}, J.}, \bibinfo{author}{{Malko}, S.},
	\bibinfo{author}{{Fedosejevs}, R.}, \bibinfo{author}{{Cayzac}, W.}, \bibinfo{author}{{Vaisseau}, X.}, \bibinfo{author}{{De Luis}, D.}, \bibinfo{author}{{Gatti}, G.}, \bibinfo{author}{{McGuffey}, C.}, \bibinfo{author}{{Bailly-Grandvaux}, M.}, \bibinfo{author}{{Bhutwala}, K.}, \bibinfo{author}{{Ospina-Bohorquez}, V.}, \bibinfo{author}{{Balboa}, J.}, \bibinfo{author}{{Santos}, J.~J.}, \bibinfo{author}{{Batani}, D.}, \bibinfo{author}{{Beg}, F.}, \bibinfo{author}{{Roso}, L.}, \bibinfo{author}{{Perez-Hernandez}, J.~A.} \& \bibinfo{author}{{Volpe}, L.}
	\newblock \bibinfo{title}{{A quasi-monoenergetic short time duration compact proton source for probing high energy density states of matter}}.
	\newblock \emph{\bibinfo{journal}{Sci. Rep.}} \textbf{\bibinfo{volume}{11}},\bibinfo{pages}{6881}
	(\bibinfo{year}{2021}).
	
	\bibitem{Pra13}
	\bibinfo{author}{{Prasad, R.}} \emph{et~al.}
	\newblock \bibinfo{title}{Thomson spectrometer–microchannel plate assembly calibration for MeV-range positive and negative ions, and neutral atoms}.
	\newblock \emph{\bibinfo{journal}{Rev. Sci. Instrum.}
	\textbf{\bibinfo{volume}{84}}, \bibinfo{pages}{053302}
	(\bibinfo{year}{2013})}.
	
	\bibitem{Fer05}
	\bibinfo{author}{{Ferrari}, A.}, 
	\bibinfo{author}{{Sala}, P.}, 
	\bibinfo{author}{{Fasso}, A.},
	\&
	\bibinfo{author}{{Ranft}, J.}
	\newblock \bibinfo{title}{{FLUKA: a multi-particle transport code}}.
	\newblock \emph{\bibinfo{journal}{CERN-2005-10}} \textbf{\bibinfo{volume}{INFN/TC$\_$05/11, SLAC-R-773}}, \bibinfo{pages}{}
	(\bibinfo{year}{2005}).
	
	\bibitem{Boh14}
	\bibinfo{author}{{Böhlen}, T.}, 
	\bibinfo{author}{{Cerutti}, F.},
	\bibinfo{author}{{Chin}, M.}, 
	\bibinfo{author}{{Fasso}, A.},
	\bibinfo{author}{{Ferrari}, A.}, 
	\bibinfo{author}{{Ortega}, P.},
	\bibinfo{author}{{Mairani}, A.},
	\bibinfo{author}{{Sala}, P.}, 
	\bibinfo{author}{{Smirnov}, G.}
	\&
	\bibinfo{author}{{Vlachoudis}, V.}
	\newblock \bibinfo{title}{{The FLUKA Code: Developments and Challenges for High Energy and Medical Applications}}.
	\newblock \emph{\bibinfo{journal}{Nuclear Data Sheets}} \textbf{\bibinfo{volume}{120}}, \bibinfo{pages}{211--214}
	(\bibinfo{year}{2014}).
	
	\bibitem{Ceg83}
	\bibinfo{author}{{Ceglio}, N.}, 
	\bibinfo{author}{{Kauffman}, R.},
	\bibinfo{author}{{Hawryluk}, A.}, 
	\&
	\bibinfo{author}{{Medecki}, H.}
	\newblock \bibinfo{title}{{Time-resolved x-ray transmission grating spectrometer for studying laser-produced plasmas}}.
	\newblock \emph{\bibinfo{journal}{Appl. Optics}} \textbf{\bibinfo{volume}{22}}, \bibinfo{pages}{318--327}
	(\bibinfo{year}{1983}).
	
	
	\bibitem{Eid86}
	\bibinfo{author}{{Eidmann}, K.}, 
	\bibinfo{author}{{Kishimoto}, T.}, 
	\bibinfo{author}{{Herrmann}, P.},
	\bibinfo{author}{{Mizui}, J.}, 
	\bibinfo{author}{{Pakula}, R.}, 
	\bibinfo{author}{{Sigel}, R.}, 
	\&
	\bibinfo{author}{{Witkowski}, S.}
	\newblock \bibinfo{title}{{Absolute soft x-ray measurements with a transmission grating spectrometer}}.
	\newblock \emph{\bibinfo{journal}{Laser Part. Beams}} \textbf{\bibinfo{volume}{4}}, \bibinfo{pages}{521--536}
	(\bibinfo{year}{1986}).
	
	\bibitem{Tau13}
	\bibinfo{author}{{Tauschwitz}, A.} \emph{et~al.}
	\newblock \bibinfo{title}{{2D radiation-hydrodynamics modeling of laser-plasma targets for ion stopping measurements}}.
	\newblock \emph{\bibinfo{journal}{High Energy Density Phys.}}
	\textbf{\bibinfo{volume}{9}}, \bibinfo{pages}{158--166}
	(\bibinfo{year}{2013}).
	
	\bibitem{Fai14}
	\bibinfo{author}{{Faik}, S.} \emph{et~al.}
	\newblock \bibinfo{title}{{Creation of a homogeneous plasma column by means of hohlraum radiation for ion-stopping measurements}}.
	\newblock \emph{\bibinfo{journal}{High Energy Density Phys.}}
	\textbf{\bibinfo{volume}{10}}, \bibinfo{pages}{47--55}
	(\bibinfo{year}{2014}).
	
	\bibitem{Bas12}
	\bibinfo{author}{{Basko}, M.~M.} \emph{et~al.}
	\newblock \bibinfo{title}{{One-dimensional study of the radiation-dominated implosion of a cylindrical tungsten plasma column}}.
	\newblock \emph{\bibinfo{journal}{Plasma Phys. Control. Fusion}}
	\textbf{\bibinfo{volume}{54}}, \bibinfo{pages}{055003(1--16)}
	(\bibinfo{year}{2012}).
	
	\bibitem{Chu05}
	\bibinfo{author}{{Chung}, H.-K.}, \bibinfo{author}{{Chen}, M.~H.},
	\bibinfo{author}{{Morgan}, W.~L.}, \bibinfo{author}{{Ralchenko}, Y.} \&
	\bibinfo{author}{{Lee}, R.~W.}
	\newblock \bibinfo{title}{{FLYCHK: Generalized population kinetics and spectral model for rapid spectroscopic analysis for all elements}}.
	\newblock \emph{\bibinfo{journal}{High Energy Density Phys.}}
	\textbf{\bibinfo{volume}{1}}, \bibinfo{pages}{3--12} (\bibinfo{year}{2005}).
	
	 \bibitem{Poye2015}
    \bibinfo{author}{Poy\'e, A. and Dubois, J.-L. and Lubrano-Lavaderci, F. and D'Humi\`eres, E. and Bardon, M. and Hulin, S. and Bailly-Grandvaux, M. and Ribolzi, J. and Raffestin, D. and Santos, J. J. and Nicola\"{\i}, Ph. and Tikhonchuk, V.}
    \newblock \bibinfo{title}{Dynamic model of target charging by short laser pulse interactions}
    \newblock \emph{\bibinfo{journal}{Phys. Rev. E}}
     \textbf{\bibinfo{volume}{92}}
     \textbf{\bibinfo{issue}{4}}
     \bibinfo{pages}{043107}
     (\bibinfo{year}{2015})
	
	\bibitem{Ram12}
	\bibinfo{author}{{Ramis}, R.}, 
	\bibinfo{author}{{Eidmann}, K.}, 
	\bibinfo{author}{{Meyer-ter-Vehn}, J.}, 
	\bibinfo{author}{{H{\"u}ller}, S.}
	\newblock \bibinfo{title}{{MULTI-fs - A computer code for laser-plasma interaction in the femtosecond regime}}.
	\newblock \emph{\bibinfo{journal}{Comput. Phys. Commun.}} \textbf{\bibinfo{volume}{183}}, \bibinfo{pages}{637--655}
	(\bibinfo{year}{2012}).

	\bibitem{MacFar04}
	\bibinfo{author}{{MacFarlane}, J.~J.}, 
	\bibinfo{author}{{Golovkin}, I.~E.}, 
	\bibinfo{author}{{Woodru}, P.~R.},
	\bibinfo{author}{{Welch}, D.~R},
	\bibinfo{author}{{Oliver}, B.~V.},
	\bibinfo{author}{{Melhorn}, T.~A.},
	\&
	\bibinfo{author}{{Campbell}, R.~B.},
	\newblock \emph{\bibinfo{Proceedings of the Third Conference on Inertial Fusion Science and Applications, Monterey, California}} \textbf{\bibinfo{volume}{2}},
	(\bibinfo{year}{2004}).

    \bibitem{Prism}
	\bibinfo{author}{ P. C. Sciences. http://www.prism-cs.com/}
	
	%----------------------------------------------------------
	% RESULTS: STOPPING CALCULATIONS
	%----------------------------------------------------------
	
	\bibitem{Zie85}
	\bibinfo{author}{{Ziegler}, J.~F.}, \bibinfo{author}{{Biersack}, J.~P.} \&
	\bibinfo{author}{{Littmark}, U.}
	\newblock \emph{\bibinfo{title}{{The Stopping and Range of Ions in Matter}}}
	(\bibinfo{publisher}{Pergamon, New York}, \bibinfo{year}{1985}).
	
	\bibitem{Mel81}
	\bibinfo{author}{{Melhorn}, T.} \emph{et~al.}
	\newblock \bibinfo{title}{{A finite material temperature model for ion energy deposition in ion‐driven inertial confinement fusion targets}}.
	\newblock \emph{\bibinfo{journal}{J. Appl. Phys.}}
	\textbf{\bibinfo{volume}{52}}, \bibinfo{pages}{6522--6532}
	(\bibinfo{year}{1981}).
	
	\bibitem{Cas13}
	\bibinfo{author}{{Casas}, D.} \emph{et~al.}
	\newblock \bibinfo{title}{{Evaluation of slowing down of proton and deuteron beams in CH2, LiH, and Al partially ionized plasmas}}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. E}}
	\textbf{\bibinfo{volume}{88}}, \bibinfo{pages}{033102}
	(\bibinfo{year}{2013}).
	
	\bibitem{Cas16}
	\bibinfo{author}{{Casas}, D.} \emph{et~al.}
	\newblock \bibinfo{title}{{Stopping power of a heterogeneous warm dense matter}}.
	\newblock \emph{\bibinfo{journal}{Laser Part. Beams}}
	\textbf{\bibinfo{volume}{34}}, \bibinfo{pages}{306--314}
	(\bibinfo{year}{2016}).
	
	\bibitem{Zyl19b}
	\bibinfo{author}{{Zylstra}, A.} \emph{et~al.}
	\newblock \bibinfo{title}{{Modified parameterization of the Li-Petrasso charged-particle stopping power theory}}.
	\newblock \emph{\bibinfo{journal}{Phys. Plasmas}}
	\textbf{\bibinfo{volume}{16}}, \bibinfo{pages}{122703}
	(\bibinfo{year}{2019}).
	
	\bibitem{BPS05}
	\bibinfo{author}{{Brown}, L.~S.}, \bibinfo{author}{{Preston}, D.~L.} \&
	\bibinfo{author}{{Singleton}, R.~L., Jr.}
	\newblock \bibinfo{title}{{Charged particle motion in a highly ionized plasma}}.
	\newblock \emph{\bibinfo{journal}{Phys. Rep.}}
	\textbf{\bibinfo{volume}{410}}, \bibinfo{pages}{237--333}
	(\bibinfo{year}{2005}).
	
	\bibitem{Ger02c}
	\bibinfo{author}{{Gericke}, D.~O.}
	\newblock \bibinfo{title}{{Stopping power for strong beam-plasma coupling}}.
	\newblock \emph{\bibinfo{journal}{Laser Part. Beams}}
	\textbf{\bibinfo{volume}{20}}, \bibinfo{pages}{471--474}
	(\bibinfo{year}{2002}).
	
	\bibitem{Ger99}
	\bibinfo{author}{{Gericke}, D.~O.} \& \bibinfo{author}{{Schlanges}, M.}
	\newblock \bibinfo{title}{{Beam-plasma coupling effects on the stopping power of dense plasmas}}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. E}}
	\textbf{\bibinfo{volume}{60}}, \bibinfo{pages}{904--910}
	(\bibinfo{year}{1999}).
	
	\bibitem{Zim90}
	\bibinfo{author}{{Zimmerman}, G.}
	\newblock \bibinfo{title}{LLNL, Report No. UCRL-JC-105616}.
	(\bibinfo{year}{1990}).
	
	\bibitem{May85}
	\bibinfo{author}{{Maynard}, G. and {Deutsch}, C.}
	\newblock \bibinfo{title}{Born random phase approximation for ion stopping in an arbitrarily degenerate electron fluid}.
	\newblock \emph{\bibinfo{journal}{J. Phys.}}
	\textbf{\bibinfo{volume}{46}}, \bibinfo{pages}{1113--1122}
	(\bibinfo{year}{1985}).
	
    \bibitem{Fau10}
	\bibinfo{author}{{Faussurier}, G.} \emph{et~al.}
	\newblock \bibinfo{title}{{Equation of state, transport coefficients, and stopping power of dense plasmas from the average-atom model self-consistent approach for astrophysical and laboratory plasmas}}.
	\newblock \emph{\bibinfo{journal}{Phys. Plasmas}}
	\textbf{\bibinfo{volume}{17}}, \bibinfo{pages}{052707}
	(\bibinfo{year}{2010}).
	
	\bibitem{Gau13}
	\bibinfo{author}{{Gauthier}, M.} \emph{et~al.}
	\newblock \bibinfo{title}{{Stopping power modeling in warm and hot dense matter}}.
	\newblock \emph{\bibinfo{journal}{High Energy Density Phys.}}
	\textbf{\bibinfo{volume}{9}}, \bibinfo{pages}{488--495}
	(\bibinfo{year}{2013}).
	
	\bibitem{Fau21}
	\bibinfo{author}{{Faussurier}, G.} \& \bibinfo{author}{{Blancard}, C.}
	\newblock \bibinfo{title}{{Friedel sum rule at finite temperature in hot dense plasmas}}.
	\newblock \emph{\bibinfo{journal}{Phys. Plasmas}}
	\textbf{\bibinfo{volume}{28}}, \bibinfo{pages}{042710}
	(\bibinfo{year}{2021}).
	
	\bibitem{Whi20}
	\bibinfo{author}{{White}, A.~J.} \& \bibinfo{author}{{Collins}, L.~A.}
	\newblock \bibinfo{title}{{Fast and Universal Kohn-Sham Density Functional Theory Algorithm for Warm Dense Matter to Hot Dense Plasma}}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. Lett.}}
	\textbf{\bibinfo{volume}{125}}, \bibinfo{pages}{055002}
	(\bibinfo{year}{2020}).
	
	\bibitem{Lom02}
	\bibinfo{author}{{Lommel}, B.}, \bibinfo{author}{{Hartmann}, W.},
	\bibinfo{author}{{Kindler}, B.}, \bibinfo{author}{{Klemm}, J.} \&
	\bibinfo{author}{{Steiner}, J.}
	\newblock \bibinfo{title}{{Preparation of self-supporting carbon thin films}}.
	\newblock \emph{\bibinfo{journal}{Nucl. Instrum. Methods Phys. Res. A}} \textbf{\bibinfo{volume}{480}}, \bibinfo{pages}{199--203}
	(\bibinfo{year}{2002}).


		
	\bibitem{Eid90}
	\bibinfo{author}{{Eidmann}, K.}, 
	\bibinfo{author}{{Kuhne}, M.}, 
	\bibinfo{author}{{Moller}, P.},
	\&
	\bibinfo{author}{{Tsakiris}, G.},
	\newblock \bibinfo{title}{{Characterization of pinhole transmission gratings}}.
	\newblock \emph{\bibinfo{journal}{J. X-Ray Sci. Technol.}} \textbf{\bibinfo{volume}{2}}, \bibinfo{pages}{259--273}
	(\bibinfo{year}{1990}).
	
	\bibitem{Vau12}
	\bibinfo{author}{{Vauzour}, B.}
	\newblock \bibinfo{title}{{Etude exp\'erimentale du transport d'\'electrons rapides dans le cadre de l'allumage rapide pour la fusion inertielle}}.
	\newblock \emph{\bibinfo{journal}{PhD Thesis, University of Bordeaux}}
	(\bibinfo{year}{2012}).
	
	\bibitem{Gus09}
	\bibinfo{author}{{Gus'kov}, S.~Y.} \emph{et~al.}
	\newblock \bibinfo{title}{{A method for calculating the effective charge of
			ions decelerated in a hot dense plasma}}.
	\newblock \emph{\bibinfo{journal}{Plasma Phys. Rep.}}
	\textbf{\bibinfo{volume}{35}}, \bibinfo{pages}{709--718}
	(\bibinfo{year}{2009}).
	
	\bibitem{Whi21}
	\bibinfo{author}{{White}, A.}, 
	\bibinfo{author}{{Collins}, L.},
	\bibinfo{author}{{Nichols},K.},\&
	\bibinfo{author}{{Hu}, S.}
	\newblock \bibinfo{title}{{Mixed Stochastic-Deterministic Time-Dependent Density Functional Theory: Application to Stopping Power of Warm Dense Carbon}}.
	\newblock \emph{\bibinfo{journal}{arXiv:2112.01638}} 
	(\bibinfo{year}{2021}). 
	
	\bibitem{Per81}
	\bibinfo{author}{Perdew}, {J. P. } 
	\&
	\bibinfo{author}{{Zunger}, A.}
	\newblock \bibinfo{title}{Self-interaction correction to density-functional approximations for many-electron systems}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. B}}
	\textbf{\bibinfo{volume}{23}}, \bibinfo{pages}{5048--5079}
	(\bibinfo{year}{1981}).
	
	\bibitem{Per96}
	\bibinfo{author}{{Perdew}, P.} 
	\bibinfo{author}{{Burke}, K.} \& \bibinfo{author}{{Ernzerhof}, M.}
	\newblock \bibinfo{title}{{Generalized Gradient Approximation Made Simple}}.
	\newblock \emph{\bibinfo{journal}{Phys. Rev. Lett.}}
	\textbf{\bibinfo{volume}{77}}, \bibinfo{pages}{3865--3868}
	(\bibinfo{year}{1996}).
	
	%\bibitem{Mal20}
	%\bibinfo{author}{{Malko}, S.}, 
	%\newblock \bibinfo{title}{{Charged particle transport in extreme state of matter}}.
	%\newblock \emph{\bibinfo{journal}{PhD Thesis, University of Salamanca}} \textbf{\bibinfo{volume}{}}, \bibinfo{pages}{}
	%(\bibinfo{year}{2020}).
	
	
	
	
	
	
	
%\bibitem{Say19}
	%\bibinfo{author}{{Sayre}, D. B.} \emph{et~al.}
	%\newblock \bibinfo{title}{{Neutron Time-of-Flight Measurements of Charged-Particle %Energy Loss in Inertial Confinement Fusion Plasmas}}.
	%\newblock \emph{\bibinfo{journal}{Physial Review Letters}}
	%\textbf{\bibinfo{volume}123}, \bibinfo{pages}{165001}
	%(\bibinfo{year}{2019}).
	
	%\bibitem{Ger02a}
	%\bibinfo{author}{{Gericke}, D.~O.} \& \bibinfo{author}{{Schlanges}, M.}
	%\newblock \bibinfo{title}{{Dense plasma temperature equilibration in the binary collision approximation}}.
	%\newblock \emph{\bibinfo{journal}{Physical Review E}}
	%\textbf{\bibinfo{volume}{65}}, \bibinfo{pages}{036418}
	%(\bibinfo{year}{2002}).
	
	%\bibitem{Hau02}
	%\bibinfo{author}{{Haun}, J.} \& \bibinfo{author}{{Schlanges}, M.}
	%\newblock \bibinfo{title}{{Electrical conductivity of nonideal carbon and zinc plasmas: Experimental and theoretical results}}.
	%\newblock \emph{\bibinfo{journal}{Physical Review E}}
	%\textbf{\bibinfo{volume}{65}}, \bibinfo{pages}{046407}
	%(\bibinfo{year}{2002}).

	%high velocity experiments
	%\bibitem{Fre15}
	%\bibinfo{author}{Frenje, J.~A.} \emph{et~al.}
	%\newblock \bibinfo{title}{Measurements of ion stopping around the bragg peak in %high-energy-density plasmas}.
	%\newblock \emph{\bibinfo{journal}{Physical Review Letters}}
	%\textbf{\bibinfo{volume}{115}}, \bibinfo{pages}{205001}
	%(\bibinfo{year}{2015}).
	
	%\bibitem{Zwi99}
	%\bibinfo{author}{{Zwicknagel}, G.} \emph{et~al.}
	%\newblock \bibinfo{title}{{	Stopping of heavy ions in plasmas at strong coupling}}.
	%\newblock \emph{\bibinfo{journal}{Physics Reports}}
	%\textbf{\bibinfo{volume}{309}}, \bibinfo{pages}{117--208}
	%(\bibinfo{year}{1999}).

	%\bibitem{Deu10}
	%\bibinfo{author}{{Deutsch}, C.} \emph{et~al.}
	%\newblock \bibinfo{title}{{Ion stopping in dense plasma target for high energy density %physics}}.
	%\newblock \emph{\bibinfo{journal}{The open plasma physics journal}}
	%\textbf{\bibinfo{volume}{3}}, \bibinfo{pages}{88 -- 115}
	%(\bibinfo{year}{2010}).
	
	%\bibitem{Wan98}
	%\bibinfo{author}{{Wang}, P.} \emph{et~al.}
	%\newblock \bibinfo{title}{{A unified self-consistent model for calculating ion stopping power in ICF plasma}}
	%\newblock \emph{\bibinfo{journal}{Physics of Plasmas}}
	%\textbf{\bibinfo{volume}{5}}, \bibinfo{pages}{2977--2987}
	%(\bibinfo{year}{1998}).
	
	%\bibitem{Rot00}
	%\bibinfo{author}{{Roth}, M.} \emph{et~al.}
	%\newblock \bibinfo{title}{{Energy loss of heavy ions in laser-produced plasmas}}.
	%\newblock \emph{\bibinfo{journal}{Europhysics Letters}}
	%\textbf{\bibinfo{volume}{50}}, \bibinfo{pages}{28--34}
	%(\bibinfo{year}{2000}).
	
	%\bibitem{Jac95}
	%\bibinfo{author}{{Jacoby}, J.} \emph{et~al.}
	%\newblock \bibinfo{title}{{Stopping of Heavy Ions in a Hydrogen Plasma}}.
	%\newblock \emph{\bibinfo{journal}{Physical Review Letters}}
	%\textbf{\bibinfo{volume}{74}}, \bibinfo{pages}{1550--1553}
	%(\bibinfo{year}{1995}).
	
	%\bibitem{Hic00}
	%\bibinfo{author}{{Hicks}, D.~G.} \emph{et~al.}
	%\newblock \bibinfo{title}{{Charged-particle acceleration and energy loss in
	%		laser-produced plasmas}}.
	%\newblock \emph{\bibinfo{journal}{Physics of Plasmas}}
	%\textbf{\bibinfo{volume}{7}}, \bibinfo{pages}{5106--5117}
	%(\bibinfo{year}{2000}).
	
	
	
\end{thebibliography}

